Beyond Universal Transformer: block reusing with adaptor in Transformer for automatic speech recognition

Transformer-based models have recently made significant achievements in the application of end-to-end (E2E) automatic speech recognition (ASR). It is possible to deploy the E2E ASR system on smart devices with the help of Transformer-based models. While these models still have the disadvantage of requiring a large number of model parameters. To overcome the drawback of universal Transformer models for the application of ASR on edge devices, we propose a solution that can reuse the block in Transformer models for the occasion of the small footprint ASR system, which meets the objective of accommodating resource limitations without compromising recognition accuracy. Specifically, we design a novel block-reusing strategy for speech Transformer (BRST) to enhance the effectiveness of parameters and propose an adapter module (ADM) that can produce a compact and adaptable model with only a few additional trainable parameters accompanying each reusing block. We conducted an experiment with the proposed method on the public AISHELL-1 corpus, and the results show that the proposed approach achieves the character error rate (CER) of 9.3%/6.63% with only 7.6M/8.3M parameters without and with the ADM, respectively. In addition, we also make a deeper analysis to show the effect of ADM in the general block-reusing method.

==> section/AISHELL_FULL_TABLE.tex <==
\begin{table}[]
\tiny
\begin{tabular}{|c|cccc|}
\hline
\multirow{2}{*}{Model} & \multicolumn{4}{c|}{WER(\%)} \\ \cline{2-5} 
& \multicolumn{1}{c|}{ctc greedy} & \multicolumn{1}{c|}{ctc prefix} & \multicolumn{1}{c|}{attention} & attention rescore\\ \hline
baseline (29Mb) & \multicolumn{1}{c|}{5.92} & \multicolumn{1}{c|}{5.91} & \multicolumn{1}{c|}{5.69} & 5.30 \\ \hline
LR (7.75Mb) & \multicolumn{1}{c|}{11.75(+98.5\%)} & \multicolumn{1}{c|}{11.75(+98.8\%)} & \multicolumn{1}{c|}{8.07(+41.8\%)} & 9.30(+75.5\%) \\ \hline
LRA-E (8.5Mb)  & \multicolumn{1}{c|}{8.38(+41.6\%/-28.7\%)} & \multicolumn{1}{c|}{8.38(+41.8\%/-29.4\%)} & \multicolumn{1}{c|}{6.63(+16.5\%/-17.8\%)} & 6.85(+29.2\%/-26.3\%) \\ \hline
\multicolumn{1}{|l|}{+ grad clip 3} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
LRA-ED  (9Mb)& \multicolumn{1}{c|}{8.55(+44.4\%/-27.2\%)} & \multicolumn{1}{c|}{8.56(+44.8\%/-27.1\%)} & \multicolumn{1}{c|}{6.97(+22.5\%/-13.6\%)} & 7.07(+33.4\%/-24.0\%) \\ \hline
LRA-D (8.25Mb) & \multicolumn{1}{c|}{10.77(+81.9\%/-8.3\%)} & \multicolumn{1}{c|}{10.77(+82.2\%-8.3\%)} & \multicolumn{1}{c|}{7.43(+30.6\%/-7.9\%)} & 8.55(+61.3\%/-8.1\%) \\ \hline
\multicolumn{1}{|l|}{+ grad clip 3} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
\end{tabular}
\end{table}

==> section/Zhijiang_wer_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{The WER of BdaR model at Non-determine scenario ASR challenge}
*: size here mean the the number of model parameters
\centering
\begin{tabular}{|c|c|c|cc|}
\hline
\multirow{2}{*}{exp} & \multirow{2}{*}{Parameters (M)*} & \multirow{2}{*}{grad clip} & \multicolumn{2}{c|}{WER (\%)}      \\ \cline{4-5} 
                     &                                     &                            & \multicolumn{1}{l|}{Dev}   & Test  \\ \hline
baseline             & 24                                  & 5                          & \multicolumn{1}{l|}{20.0}    & 24.8  \\ \hline \hline
BR      & 8                                   & 5                         & \multicolumn{1}{l|}{26.6}  & 30.4  \\ \hline
+ grad clip = 3             & 8                                   & 3                          & \multicolumn{1}{l|}{22.99} & \textbf{26.58} \\ \hline
+ 8 head             & 8                                   & 3                          & \multicolumn{1}{l|}{\textbf{21.8}}  & \textbf{26.58} \\ \hline
\end{tabular}

\label{table: zhijiang}
\end{table}
